A family of three-dimensional Virtual Elements for Hellinger-Reissner elasticity problems

We present a family of Virtual Element Methods for three-dimensional linear elasticity problems based on the Hellinger-Reissner variational principle. A convergence and stability analysis is developed. Moreover, using the hybridization technique and exploiting the information derived from this procedure, we show how to compute a better approximation for the displacement field. The numerical experiments confirm the theoretical predictions.

==> algoritmo.tex <==

\begin{figure}[H]
\begin{algorithm}
\caption{MGS algorithm}
\begin{algorithmic}[1]
\For{$i=1:\dim(\PolyTriple{k}{E}$)}
	\For{$k=1:2$} \hskip3em\Comment{re-orthoganlization procedure}	
	\State $\hat{\bs\varphi}_i^{(k)} = \hat{\bs\varphi}_i^{(k-1)}$
	\For {$j=1:i-1$} \Comment{GS orthogonalization}
	\State$\hat{\bs\varphi}_i^{(k)} = \hat{\bs\varphi}_i^{(k)}-(\hat{\bs\varphi}_i^{(k)},\bs\varphi_j)\,\bs\varphi_j$
	\EndFor%
\EndFor
	\State		$\bs\varphi_i=\hat{\bs\varphi}_i^{(k)}/||\hat{\bs\varphi}_i^{(k)}||$
	\hskip2em\Comment{Normalization}
	\EndFor
\end{algorithmic}
\end{algorithm}
\end{figure}




%
%\begin{algorithm}[H] 
%\caption{MGS algorithm with re-orthogonalization}
%\begin{algorithmic}[1]
%\For{$i=1:\dim(\PolyTriple{k}{E}$)}
%	\For{$k=1:2$} \hskip3em\Comment{re-orthoganlization %procedure}	
	%\State $\hat{\bs\varphi}_i^{(k)} = \hat{\bs\varphi}_i^{(k-1)}$
	%\For {$j=1:i-1$} \Comment{GS orthogonalization}
	%\State$\hat{\bs\varphi}_i^{(k)} = \hat{\bs\varphi}_i^{(k)}-(\hat{\bs\varphi}_i^{(k)},\bs\varphi_j)\,\bs\varphi_j$
	%\EndFor%
%\EndFor
%	\State		$\bs\varphi_i=\hat{\bs\varphi}_i^{(k)}/||\hat{\bs\varphi}_i^{(k)}||$
	%\hskip2em\Comment{Normalization}
	%\EndFor
%\end{algorithmic}
%\end{algorithm}

==> macro.tex <==
\newtheorem{thm}{Theorem}[section]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{defn}[thm]{Definition}
\newtheorem{remark}{Remark}
\newtheorem{notainterna}{Nota Interna}
% ------------------------------------------------------------------------------------------------------
% MACROS
% ------------------------------------------------------------------------------------------------------
\def\Pp{{\mathbb P}}

% \numberwithin{equation}{section}


%%%%%%% MACROS CARLO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\O}{\Omega}

\newcommand{\x}{{\mathbf{x}}}
\newcommand{\dx}{\,\mbox{d} \! \x}

\newcommand{\ds}{\,\mbox{d}s}

\newcommand{\up}{{u}_{\pi}}

\newcommand\E{{E}}  % element
\newcommand\dE{{\partial \E}}
\newcommand\DD{\mathcal D}
\newcommand\Th{{\mathcal T}_h}
\newcommand\Thi{{\mathcal T}_{h}^{i}}
\newcommand\Eh{{\mathcal E}_h}
\newcommand\Fh{{\mathcal F}_h}

\newcommand{\BB}{\mathbb{B}}
\newcommand{\hatt}{ \widehat}
\newcommand{\ttilde}{ \widetilde}

\newcommand{\calV}{ \mathcal{V}}
\newcommand{\calB}{ \mathcal{B}}
\newcommand{\calE}{ \mathcal{E}}
\newcommand{\calP}{ \mathcal{M}}
\newcommand{\calG}{ \mathcal{G}}
\newcommand{\calGb}{ \mathcal{G}^{\partial}}
\newcommand{\calGo}{ \mathcal{G}^0}
\newcommand{\rhod}{\rho_{\partial}}

\newcommand\R{\mathbb{R}}
\newcommand\C{\mathbb{C}}
\newcommand\D{\mathbb{D}}


\newcommand{\dr}{{\rm d}}
\newcommand{\EP}{P}

\renewcommand{\P}{{\mathcal P}}  % polynomials

\newcommand{\Rd}{}
\newcommand{\B}{\color{black}}

\newcommand{\VE}{V_{h|\E}}

% NEW WITH CARLO

\def\wP{\Pi}
\def\scl{(\!(}
\def\scr{)\!)}

\def\Pz{{\Pi}_{0}^\E}

%\newcommand{\MMAT}{\mathsf{M}}
%\newcommand{\RMAT}{\widehat{\mathsf{R}}}
%\newcommand{\NMAT}{\widehat{\mathsf{N}}}
%\newcommand{\DMAT}{\mathsf{D}}
%\newcommand{\PMAT}{\mathsf{P}}
%\newcommand{\IMAT}{\mathsf{I}}
%\newcommand{\KMAT}{\widehat{\mathsf{K}}}
%\newcommand{\SMAT}{\mathsf{S}}

\def\ps{p}
\def\hP{h_{\E}}
\def\hh{h}
\def\ke{{k}_{\E}}


%%%%%%%%%% MACRO CARLO %%%%%%%%%%%%%%

%%%%%%%%  BEGIN Macro %%%%%%%%%%%

%
%       grassetto   (\bftau, \bfnu,...)
%

\def\decapita#1{}
\def\grecomultibold#1#2{\grecobolddef#1\def\secondobold{#2}%
	\ifx#2\finemultibold\let\next\relax\let\secondobold\relax
	\else\let\next\grecomultibold
	\fi\expandafter\next\secondobold}

\def\grecobolddef#1{%
	\edef\dadef{bf\expandafter\decapita\string#1}%
	\expandafter\def\csname\dadef\endcsname{{\neretto #1}}}



\def\neretto#1{\setbox0=\hbox{\mathsurround=0pt$#1$}%
	\kern.02em\copy0 \kern-\wd0
	\kern-.02em\copy0 \kern-\wd0
	\raise.03em\box0 \kern.02em}
\grecomultibold\alpha\phi\beta\omega\gamma\delta\xi\sigma\tau\eta\theta\varepsilon\rho\psi\pi\varphi\varepsilon\lambda\mu\finemultibold
%
%
%      mie macro
%
%      vari simboli
%
\def\grad{\mathop{\nabla}\nolimits}
\def\grads{\mathop{{\nabla}^S}\nolimits}
\def\div{\mathop{\rm div}\nolimits}
\def\bdiv{\mathop{\bf div}\nolimits}
\def\rot{\mathop{\rm rot}\nolimits}
\def\curl{\mathop{\rm curl}\nolimits}
\def\bcurl{\mathop{\bf curl}\nolimits}
\def\tr{{\rm tr}}
\def\RE{{\bf R}}
\def\u{\mathop{\underline u}\nolimits}
\def\v{\mathop{\underline v}\nolimits}
\def\w{\mathop{\underline w}\nolimits}
\def\f{\mathop{\underline f}\nolimits}
\def\x{\mathop{\underline x}\nolimits}
\def\teps{{\bfvarepsilon}}
\def\tepsh{{\bfvarepsilon_h}}
\def\tepsc{{\bfvarepsilon_c}}
\def\tepse{{\bfvarepsilon_e}}
\def\ttau{{\bftau}}
\def\tauc{{\bftau_c}}
\def\taue{{\bftau_e}}
\def\tauh{{\bftau_h}}
%\def\sc{{\bfsigma_c}}
\def\se{{\bfsigma_e}}
\def\sh{{\bfsigma^h}}
\def\sik{{\bfsigma_i^K}}
\def\tjk{{\bftau_j^K}}
%
\def\Ls{{\rm L}}
\def\Hs{{\rm H}}
\def\Sh{{\Sigma^h}}
\def\Qh{{Q_h}}
\def\She{{\Sigma^h^e}}
\def\Shc{{\Sigma^h^c}}
%
%\let\eqno\leqno
%
%
\def\L{{\mathcal L}}
\def\T{{\mathcal T}}
\def\M{{\mathcal M}}
\def\A{{\mathcal A}}



%
\def\wbox#1;#2;{\vbox{\hrule\hbox{\vrule height#1mm\kern#2mm\vrule
			height#1mm}\hrule}}
%
%

\let\phidroit\phi
\let\phi\varphi
\let\a\alpha
\let\b\beta

\let\om\omega
\let\g\gamma
\let\G\Gamma
\let\U\Upsilon
\let\r\rho
\let\t\theta
\let\s\sigma
\let\d\partial
\let\e\varepsilon
\def\cV{{\mathcal U}}
\def\cVV{{\mathcal V}}
\def\cW{{\mathcal W}}
\def\cF{{\mathcal F}}
\def\cR{{\mathcal R}}
\def\uu{\underline{u}}
\def\vv{\underline{v}}
\def\ut{\tilde{u}}
\def\vt{\tilde{v}}
\def\wt{\tilde{w}}
\def\rlm{r_\gamma}

\def\param{\gamma}
\def\ccc{{\rm cof}}
\newcommand{\bbuht}{\hat{{\bf u}}}
\newcommand{\fffht}{\hat{{\fff}}}
\newcommand{\bbFht}{\hat{{\bbF}}}
\newcommand{\bbCht}{\hat{{\bbC}}}
\newcommand{\Jht}{\hat{{J}}}
\newcommand{\pht}{\hat{{p}}}
\newcommand{\domega}{\,{\rm d}\Omega }






% MACRO
%
\newcommand{\gmr}[1]{\mbox{\gm #1}}
\newcommand{\gmb}[1]{\mbox{\gm \bf #1}}

\newcommand{\bba}   {\mathbf{a}}
\newcommand{\bbbb}  {\mathbf{b}}
\newcommand{\bbc}   {\mathbf{c}}
\newcommand{\bbd}   {\mathbf{d}}
\newcommand{\bbe}   {\mathbf{e}}
\newcommand{\bbf}   {\mathbf{f}}
\newcommand{\bbg}   {\mathbf{g}}
\newcommand{\bbh}   {\mathbf{h}}
\newcommand{\bbk}   {\mathbf{k}}
\newcommand{\bbi}   {\mathbf{i}}
\newcommand{\bbl}   {\mathbf{l}}
\newcommand{\bbm}   {\mathbf{m}}
\newcommand{\bbn}   {\mathbf{n}}
\newcommand{\bbo}   {\mathbf{o}}
\newcommand{\bbp}   {\mathbf{p}}
\newcommand{\bbq}   {\mathbf{q}}
\newcommand{\bbr}   {\mathbf{r}}
\newcommand{\bbs}   {\mathbf{s}}
\newcommand{\bbt}   {\mathbf{t}}
\newcommand{\bbu}   {\mathbf{u}}
\newcommand{\bbv}   {\mathbf{v}}
\newcommand{\bbw}   {\mathbf{w}}
\newcommand{\bbx}   {\mathbf{x}}
\newcommand{\bby}   {\mathbf{y}}
\newcommand{\bbz}   {\mathbf{z}}
\newcommand{\bbA}   {\mathbf{A}}
\newcommand{\bbB}   {\mathbf{B}}
\newcommand{\bbC}   {\mathbf{C}}
\newcommand{\bbD}   {\mathbf{D}}
\newcommand{\bbE}   {\mathbf{E}}
\newcommand{\bbF}   {\mathbf{F}}
\newcommand{\bbG}   {\mathbf{G}}
\newcommand{\bbH}   {\mathbf{H}}
\newcommand{\bbK}   {\mathbf{K}}
\newcommand{\bbI}   {\mathbf{I}}
\newcommand{\bbL}   {\mathbf{L}}
\newcommand{\bbM}   {\mathbf{M}}
\newcommand{\bbN}   {\mathbf{N}}
\newcommand{\bbO}   {\mathbf{O}}
\newcommand{\bbP}   {\mathbf{P}}
\newcommand{\bbQ}   {\mathbf{Q}}
\newcommand{\bbR}   {\mathbf{R}}
\newcommand{\bbS}   {\mathbf{S}}
\newcommand{\bbT}   {\mathbf{T}}
\newcommand{\bbU}   {\mathbf{U}}
\newcommand{\bbV}   {\mathbf{V}}
\newcommand{\bbX}   {\mathbf{X}}
\newcommand{\bbY}   {\mathbf{Y}}
\newcommand{\bbZ}   {\mathbf{Z}}

\newcommand{\ffa}   {\mbox{\boldmath $\alpha$\unboldmath}}
\newcommand{\ffb}   {\mbox{\boldmath $\beta$\unboldmath}}
\newcommand{\ffxi}  {\mbox{\boldmath $\xi$\unboldmath}}
%\newcommand{\ffe}   {\mbox{\boldmath $\epsilon$\unboldmath}}
\newcommand{\ffe}   {\pmb{\boldsymbol{\varepsilon}}}
\newcommand{\fff}   {\mbox{\boldmath $\phi$\unboldmath}}
\newcommand{\ffg}   {\mbox{\boldmath $\gamma$\unboldmath}}
\newcommand{\ffl}   {\mbox{\boldmath $\lambda$\unboldmath}}
\newcommand{\ffk}   {\mbox{\boldmath $\kappa$\unboldmath}}
\newcommand{\ffm}   {\mbox{\boldmath $\mu$\unboldmath}}
\newcommand{\ffn}   {\mbox{\boldmath $\nu$\unboldmath}}
\newcommand{\fft}   {\mbox{\boldmath $\tau$\unboldmath}}
\newcommand{\ffth}  {\mbox{\boldmath $\theta$\unboldmath}}
\newcommand{\ffs}   {\mbox{\boldmath $\sigma$\unboldmath}}
\newcommand{\ffL}   {\mbox{\boldmath $\Lambda$\unboldmath}}
\newcommand{\ffS}   {\mbox{\boldmath $\Sigma$\unboldmath}}

\newcommand{\fourA}      {\mathbb{A}}
\newcommand{\fourB}      {\mathbb{B}}
\newcommand{\fourC}      {\mathbb{C}}
\newcommand{\fourD}      {\mathbb{D}}
\newcommand{\fourE}      {\mathbb{E}}
\newcommand{\fourF}      {\mathbb{F}}
\newcommand{\fourG}      {\mathbb{G}}
\newcommand{\fourH}      {\mathbb{H}}
\newcommand{\fourI}      {\mathbb{I}}
\newcommand{\fourL}      {\mathbb{L}}
\newcommand{\fourM}      {\mathbb{M}}
\newcommand{\fourN}      {\mathbb{N}}
\newcommand{\fourO}      {\mathbb{O}}
\newcommand{\fourP}      {\mathbb{P}}
\newcommand{\fourQ}      {\mathbb{Q}}
\newcommand{\fourR}      {\mathbb{R}}
\newcommand{\fourS}      {\mathbb{S}}
\newcommand{\fourT}      {\mathbb{T}}
\newcommand{\fourU}      {\mathbb{U}}
\newcommand{\fourV}      {\mathbb{V}}
\newcommand{\fourX}      {\mathbb{X}}
\newcommand{\fourY}      {\mathbb{Y}}
\newcommand{\fourZ}      {\mathbb{Z}}

\newcommand{\calI}       {{\mathcal{I}}}

\newcommand{\onehalf}    {\frac{1}{2}}

\newcommand{\Piext}      {\Pi^{\mbox{\scriptsize{ext}}}}
\newcommand{\Pibc}       {\Pi^{\mbox{\scriptsize{bc}}}}
\newcommand{\PiL}        {\Pi^{\mbox{\scriptsize{Lag}}}}
\newcommand{\PiHR}       {\Pi^{\mbox{\scriptsize{HR}}}}
\newcommand{\PiHW}       {\Pi^{\mbox{\scriptsize{HW}}}}
\newcommand{\PiHRm}      {\Pi^{\mbox{\scriptsize{HR,m}}}}
\newcommand{\PiHWm}      {\Pi^{\mbox{\scriptsize{HW,m}}}}
\newcommand{\bbDb}       {\bbD^{b}}
\newcommand{\bbDs}       {\bbD^{s}}
\newcommand{\bbDinv}     {\bbD^{-1}}
\newcommand{\bbFinv}     {\bbF^{-1}}
\newcommand{\bbFinvT}    {\bbF^{-T}}

\newcommand{\bbNth}      {\bbN^{\theta}}
\newcommand{\bbNbbe}     {\bbN^{\bbe}}
\newcommand{\bbNbbq}     {\bbN^{\bbq}}
\newcommand{\bbNbbu}     {\bbN^{\bbu}}
\newcommand{\bbNffe}     {\bbN^{\mbox{\boldmath \footnotesize$\varepsilon$\unboldmath}}}
\newcommand{\bbNffs}     {\bbN^{\mbox{\boldmath \footnotesize$\sigma$\unboldmath}}}
%\newcommand{\bbNffs}     {\bbN^{\ffs}}
\newcommand{\bbNp  }     {\bbN^{p}}

\newcommand{\ffthhat}    {\hat{\ffth}}
\newcommand{\bbehat}     {\hat{\bbe}}
\newcommand{\bbqhat}     {\hat{\bbq}}
\newcommand{\bbuhat}     {\hat{\bbu}}
\newcommand{\bbphat}     {\hat{\bbp}}
\newcommand{\ffehat}     {\hat{\ffe}}
\newcommand{\ffshat}     {\hat{\ffs}}

\newcommand{\thetah}     {\theta^h}
\newcommand{\bbeh}       {\bbe_h}
\newcommand{\bbqh}       {\bbq_h}
\newcommand{\bbuh}       {\bbu_h}
\newcommand{\ph}         {p_h}
\newcommand{\ffeh}       {\ffe_h}
\newcommand{\ffsh}       {\ffs_h}

\newcommand{\intB}       {\int_{\Omega}}
\newcommand{\intO}       {\int_{\Omega}}
\newcommand{\dd}         {\mbox{d}}
\newcommand{\dOmega}     {\partial \Omega}
\newcommand{\dOmegaT}    {\partial \Omega_{\theta}}
\newcommand{\dOmegabbq}  {\partial \Omega_{\bbq}}


%\def\Prime{^\prime}
%
%
%\def\LI{\hfil\break}


\def\bb #1{\underline{#1}}
\def\bbb #1{{\bb{\bb{#1}}}}
\def\Grad{\mathop{\text{grad}}\nolimits}
\def\Div{\mathop{\text{div}}\nolimits}
\def\DIV{\mathop{\text{d{\underbar{i}v}}}\nolimits}
\def\del{\mathop{\text{g{\underbar{ra}d}}}\nolimits}
\def\Del{\mathop{\text{g{\underbar{ra}d}}}\nolimits}


\def\SI{\bbb{\sigma}}
\def\TO{\bbb{\tau}}
%\def\I{\bbb{I}}
\def\DV{\bbb{D}(\bb{v})}
\def\supinf
#1#2{\mathop{\smash\sup\vphantom\inf}_{#1}\inf_{#2}}
\def\infsup
#1#2{\mathop{\smash\inf\vphantom\sup}_{#1}\sup_{#2}}
%
%\def\pointn#1{{\underline{#1}}\cdot
%	{\underline{\mathop{\smash{n}\vphantom{#1}}}}}
%%
%\def\pointv#1{{\underline{#1}} \cdot
%	{\underline{\mathop{\smash{v}\vphantom{#1}}}}}
%%
%\def\pointu#1{{\underline{#1}} \cdot
%	{\underline{\mathop{\smash{u}\vphantom{#1}}}}}
%
\def\tr{\mathop{\text{tr}}\nolimits}
\def\as{\mathop{\text{as}}\nolimits}
\def\Im{\mathop{\text{Im}}\nolimits}
\def\pointf#1{{\underline{#1}}\cdot{\underline{\mathop{\smash{f}\vphantom{#1}}}}}
\def\bo#1{\text{\bf{#1}}}


\def\hpoint#1.#2.#3{{\underline{#1}}_{#2}\cdot
	{\underline{\mathop{\smash{#3}\vphantom{{#1}_{#2}}}}}}


\def\npointp#1.#2{{\underline{#1}}\cdot
	{\underline{\mathop{\smash{#2}\vphantom{{#1}}}}}}

\def\bx{\bo{x}}
\def\by{\bo{y}}
\def\bz{\bo{z}}
\def\bw{\bo{w}}
\def\wbx{\widetilde{\bo{x}}}
\def\wby{\widetilde{\bo{y}}}
\def\wbz{\widetilde{\bo{z}}}
\def\wbw{\widetilde{\bo{w}}}
\def\bxs{\bo{x}}
\def\bys{\bo{y}}
\def\norx{\Vert\cdot\Vert_X}
\def\nory{\Vert\cdot\Vert_Y}
\def\norf{\Vert\cdot\Vert_F}
\def\norg{\Vert\cdot\Vert_G}
\def\beq{\begin{equation}}
\def\enq{\end{equation}}
\def\nv{{\mathsf v}}

% ADDED RECENTLY !!!

\def\PR{{\cal R}}
\def\tri{| \! | \! |}
\def\bfzero{{\bf 0}}
\def\xt{{\tilde x}}
\def\yt{{\tilde y}}
\def\bxt{{\tilde \bbx}}
\newcommand{\dO}    {\text{d}\Omega}
\newcommand{\dEl}    {\text{d} E}
\newcommand{\df}    {\text{d} f}
\newcommand{\de}    {\text{d} e}

\newcommand{\I}{\mathcal{I}^k}
%\def\I{\bbb{I}^k}
%\def\Ih{{\mathcal I}_h}
%\def\IE{{\mathcal I}_E}
